Degree-penalized contact processes

We study degree-penalized contact processes on Galton-Watson trees (GW) and the configuration model. The model we consider is a modification of the usual contact process on a graph. In particular, each vertex can be either infected or healthy. When infected, each vertex heals at rate one. Also, when infected, a vertex $v$ with degree $d_v$ infects its neighboring vertex $u$ with degree $d_u$ with rate $\lambda/f(d_u, d_v)$ for some positive function $f$. In the case $f(d_u, d_v)=\max(d_u, d_v)^\mu$ for some $\mu>0$, the infection is slowed down to and from high degree vertices. This is in line with arguments used in social network science: people with many contacts do not have the time to infect their neighbors at the same rate as people with fewer contacts. We show that new phase transitions occur in terms of the parameter $\mu$ (at $1/2$) and the degree distribution $D$ of the GW tree. - When $\mu\ge 1$, the process goes extinct for all distributions $D$ for all sufficiently small $\lambda>0$; - When $\mu\in(1/2, 1)$, and the tail of $D$ weakly follows a power law with tail-exponent less than $1-\mu$, the process survives globally but not locally for all $\lambda$ small enough; - When $\mu\in(1/2, 1)$, and $\mathbb{E}[D^{1-\mu}]<\infty$, the process goes extinct almost surely, for all $\lambda$ small enough; - When $\mu<1/2$, and $D$ is heavier then stretched exponential with stretch-exponent $1-2\mu$, the process survives (locally) with positive probability for all $\lambda>0$. We also study the product case $f(x,y)=(xy)^\mu$. In that case, the situation for $\mu < 1/2$ is the same as the one described above, but $\mu\ge 1/2$ always leads to a subcritical contact process for small enough $\lambda>0$ on all graphs. Furthermore, for finite random graphs with prescribed degree sequences, we establish the corresponding phase transitions in terms of the length of survival.

==> proofs_GW.tex <==
\section{Proofs of survival on Galton-Watson trees}\label{sec:survival_GW}
In this section we present proofs of survival regimes. We start with (only) global survival -- Theorem \ref{thm:max_GW}(b), then we prove Theorems \ref{thm:prod_GW} and \ref{thm:max_GW} (a) in Section \ref{sec:prod_GW_strong}.
\subsection{Max-penalty: global survival via infinite infection rays on heavy tailed GW trees}\label{sec:max_GW_weak}
To prove global survival for the max-penalty with $\mu\in(1/2,1)$ on GW trees with sufficiently fat-tailed offspring distributions, i.e., Theorem \ref{thm:max_GW}(c), we will show the existence of a (random) infinite \emph{ray} in the Galton-Watson tree on which the infection survives forever. 

\begin{definition}[Down-directed contact process]
Let $\CT$ be any (given) tree with root $\varnothing$. Consider the directed graph $\CT^{\downarrow} $ where each edge $\{u,v\}$ of $\CT$ is directed away from the root, i.e., from parent to child. Then we denote by $\CPf^{\downarrow}(\CT, \underline \xi_0)=(\underline \xi_t^{\downarrow})_{t\ge 1}$ the degree-penalized contact process in Definition \ref{def:CP} on the \emph{directed} graph $\CT^{\downarrow}$ with initial state $\underline \xi_0$.
\end{definition}
One can obtain the down-directed contact process $\CT^{\downarrow}(\CT, \underline \xi_0)$ from the graphical representation of the original $\CPf(\CT, \underline \xi_0)$ by deleting the Poisson point processes that represent infections from child to parent (i.e., upward in the tree), and leaving only those infection paths intact which only contain parent-to-child infection events. 
Hence, for every given tree $\CT$ and starting state $\underline \xi_0\in \{0,1\}^{V(\CT)}$ it holds that
\begin{equation}\label{eq:domin-downCP-CP}
\CPf^{\downarrow}(\CT, \underline \xi_0)\  {\buildrel d \over \le} \ \CPf(\CT, \underline \xi_0). 
\end{equation}
The next proposition shows global survival of $\CPf$ by showing that $\CPf^{\downarrow}$ survives with  positive probability on a Galton-Watson tree:
\begin{proposition}\label{prop:rays}
Let $\CT$ be a Galton-Watson tree with offspring distribution $D$ satisfying Definition \ref{def:power-heavy} for some $\alpha>0$ and $\Pv(D\ge 1)=1$. Suppose $\mu\in[1/2, 1)$ and $f(x,y)=\max(x,y)^\mu$, and moreover $\mu+\alpha<1$.
Then the down-directed contact process $\CPfd(\CT, \ind_{\varnothing})$  exhibits global survival with positive probability on $\CT$ for any $\lambda>0$, for almost all realizations $\CT$ of the Galton-Watson tree.
\end{proposition}
\begin{proof}
In this proof we denote by $D_v=d_v-1$ the out-degree (number of children) of the vertex in $\CT^{\downarrow}$.
Let $\CA_{\mathrm{glob}}$ be the event that $\CPf^{\downarrow}(\CT, \ind_{\varnothing})$ survives globally.
Let $\CB_K=\{\exists t_0\ge 0, \exists v\in V(\CT), \deg(v)\ge K: \xi^{\downarrow}_{t_0}(v)=1\}$ be the event that $\CPfd$ ever reaches a vertex with degree at least $K$ for a large enough $K$ decided later. This event has strictly positive probability $p_K$ with lower bound depending only on $K$, since $p_K\ge \P(D_\varnothing \ge K)>0$. 
\begin{equation}\label{eq:E1K}
\P(\CA_{\mathrm{glob}})\ge\P(\CB_K)\P(\CA_{\mathrm{glob}} \mid \CB_K),
\end{equation}
so it is enough to show that $\P(\CA_{\mathrm{glob}}  \mid \CB_K)>0$ for some large enough $K$.
Fix some constants $1<s_1<s_2$ to be chosen later.


Consider a vertex $v$ with degree $D_v= L\ge K$ in the Galton-Watson tree and let $\CN(v, [L^{s_1},L^{s_2}])$, $N(v, [L^{s_1},L^{s_2}])$ be the set and  number of children of $v$ in $\CT$ with degrees in $[L^{s_1},L^{s_2}]$, respectively. Since the children have iid degrees, $N(v,[L^{s_1},L^{s_2}]))$ is Binomially distributed with parameters  $L$  and $\P(D\in [L^{s_1},L^{s_2}])$. We bound its mean from below using \eqref{eq:heavier-power-law}. Given some $\varepsilon\in[0, \alpha(s_2-s_1)/(s_2+s_1))$, assuming $L>K_0(\varepsilon)$ so that \eqref{eq:heavier-power-law} holds,
\[ 
\begin{aligned}
\E[N(v, [L^{s_1},L^{s_2}])\mid  D_v= L]&= L\big(\P(D\ge L^{s_1})-\P(D\ge L^{s_2})\big)\\
&\ge L \Big(\frac{1}{L^{s_1(\alpha+\varepsilon)}}- \frac{1}{L^{s_2(\alpha-\varepsilon)}}\Big) = L^{1-\alpha s_1-\varepsilon s_1}(1- L^{-\alpha(s_2-s_1)+\varepsilon(s_2+s_1)})
\end{aligned}\]
By the assumption that $s_2>s_1$ and $\varepsilon<\alpha(s_2-s_1)/(s_2+s_1)$, we obtain the existence of $K_1(\varepsilon, s_2, s_1, \alpha)$ such that, the second factor on the rhs above is at least $1/2$ for all $L>K_1(\varepsilon, s_2, s_1, \alpha)\vee K_0(\varepsilon)$. Hence for all such $L$,
\begin{equation}\label{eq:ENv}
\E\big[N(v, [L^{s_1},L^{s_2}])\mid D_v= L\big) \ge L^{1-\alpha s_1-\varepsilon s_1}/2.
\end{equation}
 We now require that $s_1, \varepsilon$ is such that $1-\alpha s_1 -\varepsilon s_1>0$, then the mean tends to infinity with $L$. Using now Chernoff's bound on this Binomial random variable  we obtain that 
 \begin{equation}
 \begin{aligned}\label{eq:error-1}
 \P(\CA_{1}(v,L) | D_v=L)&:=\P\big( N(v, [L^{s_1},L^{s_2}]) > L^{1-\alpha s_1-\varepsilon s_1}/4 \mid D_v= L \big)\\ &\ge  1-\exp\big( -  L^{1-\alpha s_1-\varepsilon s_1}/48\big)=:1-\mathrm{err}_1(L).
\end{aligned} 
 \end{equation}
 Assume now that $\CPf^{\downarrow}$ has reached vertex $v$ at some time, and that $\CA_{1}(v,L)$ holds for $v$.
 Let now $\CA_2(v,L)$ be the event that $v$ infects at least one of the first $L^{1-\alpha s_1-\varepsilon s_1}/4$ many children within the set $\CN(v, [L^{s_1}, L^{s_2}])$ before healing.
We bound the complement of this event using that the degree of such a child is in the interval $[L^{s_1}, L^{s_2}]$, which gives that the infection rate from $v$ to any child $u\in \CN(v, [L^{s_1}, L^{s_2}])$ is at least $r(v,u)=\la \max(L, D_u)^{-\mu}\ge \la L^{-\mu s_2}$ (since we assumed that $s_2> s_1>1$). We obtain that
\begin{equation}\label{eq:error-2}
\begin{aligned}
    \P(\neg \CA_2(v,L) \mid v \mbox{ ever infected}, D_v=L, \CA_1(v,L) )& = \frac{1}{1+\sum_{u_i \in \CN(v, [L^{s_1}, L^{s_2}], i \le L^{1-\alpha s_1-\varepsilon s_1}/4 }r(v,u_i)} \\&\le \frac{1}{1+\lambda L^{1-\alpha s_1-\mu s_2-\varepsilon s_1}/4}
    \\
    &\le 8\lambda^{-1}L^{-(1-\alpha s_1-\mu s_2-\varepsilon s_1)}=:\mathrm{err}_2(L),
    \end{aligned}
\end{equation}
where we used that $L$ is sufficiently large, and the assumption that $1-\alpha s_1-\mu s_2-\varepsilon s_1>0$ to obtain the last line. This assumption can be satisfied with $s_2>s_1>1$ and $\varepsilon>0$ small enough whenever $1-\alpha-\mu>0$, which is true since we assumed $\alpha+\mu<1$. Also note that it cannot be satisfied when $\alpha+\mu\ge 1$.

We use the error bound in \eqref{eq:error-2} repeatedly. 
Let now $v_0$ be the first vertex reached by $\CPf^{\downarrow}$ with degree at least $K$ in the event $\CB_K$ in \eqref{eq:E1K}, and let $D_{v_0}$ denote its random degree. We now define a random infection ray $(v_0, v_1, \dots, v_m, v_{m+1} \dots)$ recursively. Suppose we already defined $(v_0, \dots, v_m)$ for some $m\ge 0$, and their degrees $(D_{v_0}, \dots, D_{v_m})$. 
We now check whether the event $\CA_1(v_m, D_{v_m})\cap \CA_{2}(v_m, D_{v_m})$ holds, and if so, then we choose any vertex $v_{m+1}\in \CN(v_m, [D_{v_m}^{s_1}, D_{v_m}^{s_2}])$ that is infected by $v_m$ before $v_m$ heals.
We now obtain the existence of an infinite ray by taking the limit of the nested sequence of events: 
\[ 
\begin{aligned}
\P\big( (v_0, \dots, v_m, \dots) \mbox{ exists}\big)&=\lim_{m_0\to \infty}  \P\Big(\cap_{m\le m_0} \{v_{m+1} \mbox{ exists}\}\Big)\\
&=
\lim_{m_0\to \infty} \prod_{m=0}^{m_0} \P\Big( v_{m+1} \mbox{ exists} \mid (v_0, \dots, v_{m}) \mbox{ exists}\Big),
\end{aligned}\] We denote by $\CF_{m}$ the sigma-algebra generated by $\cup_{i\le m-1}\{\CA_1(v_i, D_{v_i}), \CA_2(v_i, D_{v_i}), v_i, D_{v_i}\} \cup \{v_{m},D_{v_m}\}$. I.e., we reveal the degree and existence of $v_m$, but not whether $\CA_1(v_m, D_{v_m}) \cap \CA_2(v_m, D_{v_m})$ holds since those events already give $v_{m+1}$. Using this sigma-algebra, we can use the Markov property of $\CPf^{\downarrow}$, lower bound the probability of existence of $v_{0}$ by $\P(\CB_K)$, and that of $v_{m+1}$ by the conditional probability of $\CA_1(v_m, D_{v_m})\cap \CA_{2}(v_m, D_{v_m})$ to obtain
\begin{equation}\label{eq:infinite-ray}
 \begin{aligned}
\P\big( (v_0, \dots, v_m, \dots)& \mbox{ exists}\big) \ge \lim_{m_0\to \infty}\P(\CB_K)\E\Bigg[\prod_{m=0}^{m_0} \P\Big(\CA_1(v_{m}, D_{v_m}) \cap \CA_2(v_m, D_{v_m})\mid \CF_{m}\Big)\bigg] \\
& \ge\P(\CB_K)\lim_{m_0\to \infty}\Bigg[\prod_{m=1}^{m_0} \P\Big(\CA_1(v_m, D_{v_m}) \cap \CA_2(v_m, D_{v_m})\mid v_{m} \mbox{ ever infected}, D_{v_{m}}\Big)\Bigg]
\end{aligned}
\end{equation}
Observe that now the calculations in \eqref{eq:error-1} and \eqref{eq:error-2} apply, and the $m$th factor is, conditionally on $D_{v_m}$, at least 
$1-\mathrm{err}_1(D_{v_m})-\mathrm{err}_2(D_{v_m})$.
We inductively show that the $m$th factor in the product above is at least 
\begin{equation}\label{eq:vm-degree}
 1-\mathrm{err}_1(K^{s_1^m})-\mathrm{err}_2(K^{s_1^m}),
\end{equation}
by showing that $D_{v_m}\ge K^{s_1^m}$ whenever $v_m$ exists. Monotonicity of $\mathrm{err}_1(L)+\mathrm{err}_2(L)$ in $L$ then immediately yields \eqref{eq:vm-degree}. Since we assumed $D_{v_0}\ge K=K^{s_1^0}$, the induction starts. Assume now that $v_{m-1}\ge K^{s_1^{m-1}}$. Then per definition, (see \eqref{eq:error-2}),  $D_{v_m}\in [D_{v_{m-1}}^{s_1}, D_{v_{m-1}}^{s_2}]$. Using now the induction hypothesis immediately gives  \eqref{eq:vm-degree}.

Hence, we return to \eqref{eq:infinite-ray}, for a.e. realization in the conditional expectation the lower bound in  \eqref{eq:vm-degree} holds, hence, 
\begin{equation}\label{eq:infinite-ray-2}
\begin{aligned}
\P\big( (v_0, \dots, v_m, \dots) \mbox{ exists}\big)&\ge \P(\CB_K)\prod_{i=1}^{\infty} ( 1-\mathrm{err}_1(K^{s_1^m})-\mathrm{err}_2(K^{s_1^m}))\\
&\ge \P(\CB_K)\Big( 1- \sum_{m=0}^\infty \mathrm{err}_1(K^{s_1^m})+\mathrm{err}_2(K^{s_1^m}) \Big)\\
\end{aligned}\end{equation}
Using the values of $\mathrm{err}_1(K^{s_1^m})+\mathrm{err}_2(K^{s_1^m})$ from \eqref{eq:error-1}, \eqref{eq:error-2}, given that 
\begin{equation}\label{eq:s1-s2}
    1<s_1<s_2, \qquad 1-\alpha s_1-\mu s_2-\varepsilon s_1>0, \qquad 1-\alpha s_1 - \varepsilon s_1>0,
\end{equation}
the sum on the right hand side is summable in $m$, and both terms decrease faster then geometric in $m$, hence they are dominated by a constant times their first term:
\begin{equation}\label{eq:summed-errors}
\begin{aligned}
\sum_{m=0}^{\infty}\exp(- K^{s_1^m(1-\alpha s_1 - \varepsilon s_1)}/48)&+\sum_{m=0}^{\infty}8\lambda^{-1} K^{-s_1^m(1-\alpha s_1-\mu s_2-\varepsilon s_1)}\\&\le C \exp(-K^{1-\alpha s_1 - \varepsilon s_1}/48) + C \la^{-1} K^{-(1-\alpha s_1-\mu s_2-\varepsilon s_1)}.
\end{aligned}\end{equation}
One can check that the system of inequalities in \eqref{eq:s1-s2} is solvable whenever $1-\alpha-\mu>0$. Namely, choose first $1<s_1< s_2$ close enough to $1$ so that 
$1-\alpha s_1-\mu s_2>0$ holds. Choose then $\varepsilon>0$  small enough so that \eqref{eq:ENv} and \eqref{eq:s1-s2} hold as well, and finally one can set $K$ sufficiently large so that all inequalities above are valid. 
In particular, given now any $\la>0$ (i.e., small), one can choose $K$ sufficiently large so that the sum in \eqref{eq:summed-errors} is at most $1/2$, and then we obtain in \eqref{eq:infinite-ray-2} that an infinite infection ray exists with probability at least $\P(\CA_K)/2$, which is strictly positive. Hence, global survival occurs with strictly positive probability, whenever $\alpha+\mu<1$, finishing the proof.
\end{proof}



\subsection{Product penalty: local survival using a row of star-graphs when $\mu<1/2$}\label{sec:prod_GW_strong}

We will prove local survival of $\CPf$ (for both product and maximum penalty) when $\mu\in [0, 1/2)$ on the Galton-Watson tree, with at last stretched exponential offspring distributions, i.e., Theorem \ref{thm:prod_GW} in multiple steps. 

The idea is the following: As a direct consequence of known results, in Claim \ref{claim:star} we prove that when $\mu<1/2$, the infection survives on a star-graph of degree $K$, which consist of a degree-$K$ vertex and its degree-$1$ neighbors, for a time $T_K=\exp(\Theta(\lambda^2 K^{1-2\mu}))$ with probability very close to $1$. Moreover, throughout this time the star will be \emph{infested}, by which we mean that a sufficiently high fraction of its vertices are infected. 

We then show that a star-graph that is infested for time $T_K$, sends the infection through a path of length $\ell$ to another such star-graph with probability close to $1$ if and only if $\ell= o(\log T_K)$. Hence we need that $\ell=o(K^{1-2\mu})$ so that the infection successfully infests another star-graph. 

Let $H_{K, \ell(K)}$ be a graph that consists of a one-ended infinite row of star-graphs of degree $K$, $(v_1,v_2,  \dots)$, with paths of length $\ell(K)=o(K^{1-2\mu})$ between two consecutive stars. We show that the degree-penalized contact process survives forever on $H_{K, \ell(K)}$ with positive probability, as long as $K$ is sufficiently large compared to $\lambda$. We do this by mapping the process on $H_{K, \ell(K)}$ to a discrete time analog of the contact process on $\N_+=\{1,2,\dots\}$ corresponding to the infinite row of star-graphs $(v_1, v_2, \dots)$.

We then show that $H_{K, \ell(K)}$ can be embedded almost surely in a Galton Watson tree $\CT_D$ in a way that in the embedding, every vertex in $H_{K, \ell(K)}$ has degree at most $M$ times its degree in $H_{K, \ell(K)}$. This only changes $\lambda$ in the arguments above by a constant factor, i.e, to $\tilde\lambda:=\lambda/M^{2\mu}$, so if $\CPf$ survives on $H_{K, \ell(K)}$ whenever $K$ is sufficiently large, then the same is true for $\mathrm{CP}_{f, \tilde\lambda}$ by increasing $K$ if necessary. For the embedding to be possible, the tail of $D$ must be heavier than stretched exponential with stretch-exponent $1-2\mu$, in the sense of Definition \ref{def:stretched-heavy}, which is the mildest condition possible for this proof to work.

\subsubsection{Embedding stars in the Galton-Watson tree}\label{sec:embedded_stars}
We now make the former outline precise, starting with the definition of the infinite row of star-graphs and the embedding that does not increase degrees too much.  
\begin{definition}[Infinite path of stars and $M$-embedding]\label{def:M-embedding}
Given two integers $K, \ell\ge 1$, let $H=H_{K,\ell}$ be an infinite graph defined as follows: consider an infinite path $(v_1, \CP_1, v_2, \CP_2, \dots, v_i, \CP_i, v_{i+1}, \dots)$, where for all $i\ge 1$ the  paths $\CP_i=(u_1^{\sss{(i)}}, \dots, u_\ell^{\sss{(i)}})$ have length $\ell$, and where each $v_i, i\in \N$ 
has additionally $K$ neighbors $w_1^{\sss{(i)}}, \dots, w_{K}^{\sss{(i)}}$, each with $\deg_H(w_j^{\sss{(i)}})=1$ that we call leaves.
We call $K$ the star-degree of $H_{K, \ell}$ and $\ell$ the connecting-path length, which might depend on $K$. See Figure \ref{fig:Hkl}.

We say that $H=H_{K,\ell}$ is (degree-factor) $M$-embedded in a graph $G$ if $G$ contains $H_{K,\ell}$ as subgraph, and for all vertices $v\in H_{K, \ell}\subseteq G$  it holds that 
\begin{equation}\label{eq:factor-M} \frac{\deg_G(v)}{\deg_H(v)}\le M. \end{equation}
\end{definition}

\begin{figure}[h]
\includegraphics[scale=1]{Hkl.pdf}
\caption{The graph $H_{K,\ell(K)}$.}
\label{fig:Hkl}
\end{figure}
 
The next lemma shows that for large $K$, $H_{K,\ell}$ can be $M$-embedded almost surely into a Galton-Watson tree $\CT$ with offspring distribution $D$. The proof reveals that the tail of $D$ determines the minimal $\ell=\ell(K)$ that is possible for the embedding to hold almost surely.
\begin{lemma}\label{lem:embedded_stars}
Let $\CT$ be a Galton-Watson tree with degree distribution $D$ so that the tail of $D$ is heavier  than stretched exponential with stretch-exponent $1-2\mu$, in the sense of Definition \ref{def:stretched-heavy}, along the infinite sequence $(K_i)_{i\ge 1}$, and prefactor $g(K)\to 0$ as $K\to 0$.
 Then there exists a constant $M\ge 1$, such that $H_{K, \ell(K)}$ can be $M$-embedded in $\CT$ for all sufficiently large $K$ such that $2K\in \{K_i, i\ge 1\}$, for almost all realizations of $\CT$, whenever
 \begin{equation}\label{eq:ellK}
 \ell(K)\ge 2^{1-2\mu} \sqrt{g(2K)} K^{1-2\mu} = o(K^{1-2\mu}).
 \end{equation}
\end{lemma}
\begin{proof}
First, fix some small constant $\eps>0$ decided later. Let $\E[D]:=q>1$, and define $D_{M}:=D\ind_{D< M}$, i.e., the distribution where $\P(D_{M}=0)=\P(D=0)+\P(D\ge M)$ and $\P(D_{M}=k)=\P(D=k)$ for all $k\in[1,M)$.
Given $\varepsilon>0$, we choose $M>2$ such that both of the following inequalities hold:
\begin{equation}\label{eq:qM} 
\begin{aligned}
q_M:=\E[D_M]&=\E[D\ind\{D< M\}]\ge \E[D]-\eps>1+2\varepsilon\\
\P(D < M) &\ge 1-\varepsilon.
\end{aligned}
\end{equation}

It is clear that $D_{M}$ can be coupled to $D$ such that $\P(D_{M} \le D)=1$, and this embedding can be done for each vertex of the original Galton Watson tree $\CT$, obtaining a sub-forest $\CF_{M}$ of $\CT$. The embedding can be done by first sampling $D_v \sim D$ many children for each vertex $v$, and then accepting the number of offspring as it is when $D_v$ is between $0$ and $M-1$, but   setting the degree of $v$ in $\CF_M$ to be $0$ when $D_v\ge M$.  We will denote the distribution of a single tree in $\CF_M$ by $\CT_M$, which is a branching process with offspring distribution $D_M$. 

 Define the event, for $2K\in\{K_i\}_{i\ge 1}$,
\[ \CA_1:=\{ \exists v\in \CT: D_v = 2K\}.\]
Since we assumed $\P(D=0)=0$, $\CT$ survives almost surely and so $\P(\CA_1)=1$.
Take then the vertex $v\in \CT$ that is closest to the root $\varnothing$ and has $D_v =2K$, and set it to $v_1$ in $H_{K, \ell}$ of the embedding. Clearly $v_1$ then satisfies \eqref{eq:factor-M} since its degree in $\CT$ is $2K\le MK$ by our assumption that $M\ge 2$.

 Similarly as in the proof of Proposition \ref{prop:rays} below \eqref{eq:E1K}, let $\CN(v, [a,b]), N(v, [a,b])$ denote the set and number of children of a vertex $v\in \CT$ with offspring in the interval $[a,b]$. 
Consider now the event $\CA_{\text{child}}(v_1):=\{ N(v_1, [0,M) ) \ge K+1\}$. Since $D_{v_1}= 2K$ per assumption, and the children of $v_1$ have iid degrees, using \eqref{eq:qM}, each of these children has offspring less than $M$ with probability at least $1-\varepsilon$. Hence, using the concentration of Binomial random variables (e.g. a Chernoff's bound), whenever $\varepsilon<1/8$ (which we safely assume), for all $K$ sufficiently large,
\begin{equation}\label{eq:M-children}
\P\big(\CA_{\text{child}}(v_1)\big) =\P\big(N(v_1, [0,M) ) \ge K+1\big)\ge \P( \ \mathrm{Bin}(2K, 1-\eps) > K) \ge 1-\e^{-K/12}.
\end{equation}

On the event $\CA_{\text{child}}(v_1)$, label the first $K+1$  children in $\CN(v_1, [0,M))$ as $w_1,w_2,\ldots,w_{K+1}$. 
Including the edge towards $v_1$, the total degree of any of these vertices in $\CT$ is at most $M$, satisfying thus the degree factor $M$ in \eqref{eq:factor-M}. So, $v_1$ and any $K$ out of the children $w_1, \dots, w_{K+1}$ may serve as the embedding of $w_1^{\sss{(1)}}, \dots, w_{K}^{\sss{(1)}}$ of $H_{K, \ell}$, and any one of these children may take the role of $u_1^{\sss{(1)}}$ of the path $\mathcal P_1$ in $H_{K, \ell}$.

 From each of these vertices $w_i$ we start the (embedded) branching process $\CT_{M}(w_i)\subseteq \CT(w_i)$ with offspring distribution $D_{M}$. Let the number of descendants of $w_i$ in $\CT_{M}(w_i)$ in generation $\ell$  (that is, of distance $\ell$ from $w_i$) be $Z^{(i)}_{\ell}$ for each $\ell\ge 1$. It is well-known that $W^{(i)}_{\ell}:=Z^{(i)}_{\ell}/q_M^{\ell}$ is a martingale for each $i$ \cite{athreya2004branching}, and that $\lim_{\ell\to\infty}W^{(i)}_{\ell}=W^{(i)}_{\infty}$ exists a.s. Since $\E[D_M]=q_M>1+2\varepsilon$, this branching process is supercritical, and because $D_{M}$ is bounded by $M$, the Kesten-Stigum Theorem gives that $\eta:=\P(W^{(i)}_{\infty}\ne 0)>0$ is the probability that the corresponding branching process $\CT_M$ survives indefinitely. It follows then that, for any $i$,
\[
\lim_{\ell\to\infty}\P(Z^{(i)}_{\ell}\ge (q_M-\eps)^{\ell})=
\lim_{\ell\to\infty}\P\left(\frac{Z^{(i)}_{\ell}}{q_M^{\ell}}\ge \left(\frac{q_M-\eps}{q_M}\right)^{\ell}\right)=\P(W^{(i)}_{\infty}> 0)=\eta.
\]
By \eqref{eq:qM}, $q_M-\varepsilon>1+\varepsilon$ and consequently, there exists a (deterministic) $\ell_0$ only depending on $D_{M}$ (but not on $K$) such that for all $\ell>\ell_0$ we have
\begin{equation}\label{eq:E1}
\P(\CB_i):=\P(Z^{(i)}_{\ell}\ge (q_M-\eps)^{\ell})\ge\eta/2.
\end{equation}
Denote the set of individuals in the  $\ell$-th generation of $w_i$ by $\mathcal{G}^{(i)}_{\ell}$ for each $i=1,2,\ldots,K$, and let $\mathcal{G}_{\ell}=\cup_{i=1}^K\mathcal{G}^{(i)}_{\ell}$. 
Since $(w_i)_{i\le K}$ are siblings, $\CG_\ell$ is embedded in $\CT$ also in the same (possibly other than $\ell$) generation.
We now return to the original branching process $\CT$ for a single generation.
For each $v\in\mathcal{G}_{\ell}$ consider i.i.d. copies $D_v$ of $D$ (that is, without the truncation at $M$ used so far), and define the events for $i\le K$:
\begin{align}
\widetilde\CB_i&:=\{\exists u_{\sss{(i)}}\in\mathcal{G}^{(i)}_{\ell}:\ D_{u_{\sss{(i)}}}= 2K\}\label{eq:Fi}
\end{align}
for each $i=1,\ldots,K+1$. 
By \eqref{eq:E1} we have $\P(\CB_i)\ge \eta/2$.
Furthermore, since on the event $\CB_i$
\begin{align}
\P(\neg \widetilde\CB_i\mid \CB_i)&\le \big(1-\P( D= 2K)\big)^{(q_M-\eps)^{\ell}}\nonumber\\
&\le \exp\Big(-\P(D=2K)(q_M-\eps)^{\ell}\Big).\nonumber
\end{align}
Since we have assumed $2K\!\in\!\{K_i\}_{i\ge 1}$ in Definition \ref{def:stretched-heavy}, we can use the bound $\P(D\!=\!2K)\ge\exp(-g(2K) (2K)^{1-2\mu})$ for the function $g(2K)\to 0$ as $K\to 0$ in Definition \ref{def:stretched-heavy}. Hence, $g(2K)=o(\sqrt{g(2K)})$ but at the same time $\sqrt{g(2K)}\to 0$ as $K\to \infty$. We then also use that $q_M-\eps>1+\eps$ by assumption, and so by choosing $\ell=\ell(K)\ge\sqrt{g(2K)} (2K)^{1-2\mu}$, one can compute that $(2K)^{1-2\mu}(\sqrt{g(2K)}\log(q_M-\eps)-g(2K))\to \infty$ and so for all sufficiently large $K$ it holds that 
\begin{equation}\label{eq:FEi}
\begin{aligned}
\P(\neg \widetilde\CB_i\mid \CB_i)&\le\exp\Big(-\e^{-g(2K) (2K)^{1-2\mu}}(q_M-\eps)^{\ell(K)}\Big)\\
&\le \exp\big(-\e^{ (2K)^{1-2\mu} ( \sqrt{g(2K)}\log(q_M-\eps) - g(2K))}\big) \le 1/2.
\end{aligned}
\end{equation}
Combining \eqref{eq:E1} and \eqref{eq:FEi} yields
\begin{align}
\P(\widetilde\CB_i)\ge\P(\CB_i)\cdot\P(\widetilde\CB_i\mid \CB_i)
\ge
(\eta/2)\cdot (1/2) \ge \eta/4. 
\end{align}
Now we define the event that at least two events $\widetilde\CB_i, \widetilde\CB_j$ happen for $v_1$:
\begin{align}
\widetilde\CA(v_1)&:=\{\exists i, j:\  i\neq j : \widetilde\CB_i\cap \widetilde\CB_j \mbox{ holds}\}.\label{eq:defF}
\end{align}

Now consider the number of indices $i\le K+1$ for which $\widetilde\CB_i$ holds. 
By \eqref{eq:Fi}, on the event $\CA_{\text{child}}(v_1)$ in \eqref{eq:M-children}, this number stochastically dominates a binomial random variable with parameters $K+1$ and $\eta/4$. Hence, by the definition of $\widetilde\CA(v_1)$ in \eqref{eq:defF}, it holds for some constant $c(\eta)>0$ that
\begin{equation*}
\P(\widetilde\CA(v_1)\mid \CA_{\text{child}}(v_1))\ge \P(\mathrm{Bin}(K+1, \eta/4)\ge 2)
=1-(1-\eta/4)^{K+1}-K(\eta/4)(1-\eta/4)^{K} \ge 1-\e^{-c(\eta) K}.
\end{equation*}
Combining this with \eqref{eq:M-children}, we obtain that for all sufficiently large $K$,
\begin{equation}\label{eq:2-children}
\P(\CA_{\text{child}}(v_1)\cap \widetilde\CA(v_1)) \ge 1- \e^{-c(\eta) K} - \e^{-K/12}\ge 1-\varepsilon.
\end{equation}
On the event $\tilde\CA(v_1)\cap \CA_{\text{child}}(v_1)$, there are two vertices $v_{2,1}, v_{2,2}$ such that their most recent common ancestor is the starting vertex $v_1$, and $\deg(v_{2,1}),\deg(v_{2,2})=2K $, and $d_G(v_{1},v_{2,1})=d_G(v_1,v_{2,2})=\ell(K) \ge \sqrt{g(2K)}(2K)^{1-2\mu}$ with $\ell(K)=o(K^{1-2\mu})$,
and the paths $\mathcal{P}_{1,1}, \mathcal P_{1,2}$ joining  $v$ with $v_{2,1}$ and $v_{2,2}$ respectively are edge-disjoint with all internal vertices having degree at most $M$. 
Observe that $(v_1, \mathcal P_{1,1}, v_{2,1})$ and $(v_1,  \mathcal P_{1,2}, v_{2,2})$ both serve as a factor $M$-embedding of the vertices in $(v_1, \mathcal P_1, v_2)$ in $H_{K, \ell(K) }$, hence we may choose any of them for the embedding. Further, the vertices $v_{2,1}$ and $v_{2,2}$ have degree $2K$ in $\CT$, hence, using the argument betwee \eqref{eq:M-children} and \eqref{eq:defF}, one can repetitively apply the procedure of checking whether the events $\CA_{\text{child}}(\cdot) \cap \tilde\CA(\cdot)$ hold for these vertices, and the vertices then found by either $\CA_{\text{child}}(v_{2,1}) \cap \tilde\CA(v_{2,1})$ or $\CA_{\text{child}}(v_{2,2}) \cap \tilde\CA(v_{2,2})$ may all serve  as the embedding of the path $\mathcal P_2$ and $v_3$, and so on. 

 We thus consider an auxiliary ``renormalised'' branching process. We say that $v_1$ has $2$ children (in this case $v_{2,1}, v_{2,2}$) with probability (at least) $1-\varepsilon$ in \eqref{eq:2-children} and $0$ otherwise. Observe that the path leading to any vertex in generation $j$ of this branching process serves as an $M$-embedding of $(v_1, \CP_1, v_2, \dots, \CP_{j-1}, v_j)$.
 This renormalised branching process is supercritical. Hence, it survives with positive probability, giving that the $M$-embedding of the infinite graph $H_{K, \ell(K)}$ exists in $\CT$, starting from $v_1$, with positive probability. 
Kolmogorov's 0-1 law finishes the proof that $\CT$ then has a proper $M$-embedding of $H_{K, \ell(K)}$ somewhere in $\CT$ with probability $1$.
\end{proof}
We now define star-graphs (subgraphs of $H_{K, \ell}$) and the notion of infested stars.
\begin{definition}
A \emph{star-graph} $S$ of degree $K$ is a graph which consists of one vertex $v$ of degree $\deg_S(v)=K$ (its center) and its $K$ neighbors $(w_i)_{i\le K}$, each of degree $\deg_S(w_i)=1$ that we call leaves. 
Consider the classical contact process with infection rate $r$ on $S$.
We will call such a star $r$-\emph{infested} at some time $t$ by the contact process if at least $r K/(16e^2)$ of its leaves are infected.
\end{definition}

The next claim adapts \cite[Lemma 3.1]{MVY2013} to the degree-penalized contact process on $S$. The claim shows that  starting with only the center infected, a star-graph is $\la K^{-\mu}$-\emph{infested} for a time interval of length $T_K\ge \exp(c r^2 K)= \exp(c\lambda^2 K^{1-2\mu})$ with high probability, and during this time-interval the center vertex $v$ is infected more than half of the time.
Writing $r$ for the rate of infection of the classical contact process on a star-graph, \cite[Lemma 3.1]{MVY2013} holds under the condition that $r^2 K$ is uniformly bounded away from $0$. Since in the degree-penalized CP, the rate across the edges of the star-graph is $r=\lambda K^{-\mu}$, we shall require that $\lambda^2 K^{1-2\mu}$ is uniformly bounded away from $0$:
\begin{claim}[Lemma 3.1 of \cite{MVY2013} adapted]\label{claim:star}
Assume $\mu<1/2$, $\lambda<1$. Consider a star-graph $S$ of degree $K$ with center $v$. 
Let $\xi_t$ denote the contact process $\mathrm{CP}$ on $S$ where   $r(v,u)=r(u,v)=\la /K^\mu$,
 Then there exists a constant $c_1>0$ such that
 \begin{equation}\label{eq:star-i}\P\left(|\underline\xi_1|\ge\lambda K^{1-\mu}/(4e)\mid \xi_0(v)=1\right)\ge (1-e^{-c_1\lambda K^{1-\mu}})/e;
 \end{equation}
Further, if $\lambda^2 K^{1-2\mu}>32e^2$, then \begin{equation}\label{eq:star-ii}
\P\Big(\underline\xi_{\exp\{c_1\lambda^2 K^{1-2\mu}\}}\ne\emptyset\ \Big|\  |\underline\xi_0|\ge\lambda  K^{1-\mu}/(8e)\Big)\ge 1-e^{-c_1\lambda^2 K^{1-2\mu}}=:1-\mathrm{err}_{\lambda,K}.
\end{equation}
Moreover, let $T_K:=\exp(c_1\lambda^2 K^{1-2\mu})$. Then
\begin{equation}\label{eq:star-iii}
\P\left(S\text{ is $\lambda K^{-\mu}$-infested for all } t\in\left[0,T_K\right] \mbox{and} \int_{0}^{T_K} \xi_t(v) \ge T_K/2\ \Big|\  |\xi_0|\ge\lambda  K^{1-\mu}/(8e)\right)\ge 1-\mathrm{err}_{\lambda,K}.
\end{equation}
\end{claim}

The proof of Claim \ref{claim:star} is very similar to \cite[Lemma 3.1]{MVY2013}, therefore we include it in the Appendix.

\subsubsection{Contact process on an infinite line of stars}\label{sec:spread_between_stars}
We continue by studying the spread of the infection on $H_{K, \ell(K)}$. In particular, we prove that the probability that an infested star passes on the infestation to a neighboring star in $H_{K, \ell(K)}$ can be made arbitrarily close to $1$ with the right choice of the parameters.
\begin{claim}\label{claim:spread_between_stars} 
For each fixed small $\lambda>0$ and $\delta>0$ there is a $K_{\lambda, \delta}$ such  that the following holds for all $K\ge K_{\lambda, \delta}$. Consider the degree-penalized contact process $\mathrm{CP}_{f,\lambda}$ on $H_{K, \ell(K)}$ with $f=(xy)^{\mu}$ for some $\mu<1/2$.
Consider two consecutive stars $v_i, v_{i+1}$ in $H_{K, \ell(K)}$ in Definition \ref{def:M-embedding}, with $\ell(K)=o(K^{1-2\mu})$, and let $T_K:=\exp(c_1\lambda^2 K^{1-2\mu})$ from Claim \ref{claim:star}.
Suppose that $v_i$ is $\lambda K^{-\mu}$-infested at some time $t_0$. Then at time $t_0+T_K$, $v_{i+1}$ is $\lambda K^{-\mu}$-infested with probability at least $1-\delta$. 
\end{claim}
\begin{proof}
In Definition \ref{def:M-embedding}, we denoted the vertices on the path $\CP_i$ connecting $v_i$ to $v_{i+1}$ by $u_1^{\sss{(i)}}, u_2^{\sss{(i)}}, \dots u_{\ell}^{\sss{(i)}}$. In this proof we will omit the superscript.  Also, $c>0$ is a constant whose value can be made specific but may vary even within line.  Further, $|\cdot|$ means the Lebesgue measure of a set in $\R$.
   We define the event and bound its probability from below using \eqref{eq:star-iii}:
  \begin{equation}\label{eq:localtime}
\P(\CA_1(v_i)) :=\{ v_i \mbox{ is }\lambda K^{-\mu}\mbox{-infested for all } t\in [t_0, t_0+T_K]\} \ge 1-\e^{c_1 \lambda^2 K^{1-2\mu}}\ge 1-\delta/8,
\end{equation}
whenever $K\ge \log(8/\delta) \lambda^{-2/(1-2\mu)}/c_1=:K_0(\delta)$.
For some $m_K$ and $t_K$ to be determined later, partition the time interval $[t_0, t_0+T_K]$ into  $m_K$ disjoint intervals of length $t_K$, denoted by $J_1, \dots J_{m_K}$, with $m_K= \lfloor T_K/t_K\rfloor$.
Since $v_i$ is infested at time $t\in [t_0, t_0+T_K]$, the proof of Claim \eqref{claim:star} reveals that $\xi_t(v_i)$ is stochastically dominating a two-state Markov chain on $\{0,1\}$ with transition rate $q_{0,1}=\lambda^2K^{1-2\mu}/(16\e^2)$ and $q_{1,0}=1$. 
For each interval $J_j=[J_j^-, J_j^+)$, let $\tau_j$ denote the first time in $J_j$ when $\xi_t(v_i)=1$. Define then the event that 
\begin{equation}\label{eq:JJ}
\CA_2(J_j):=\{\tau_j \le 1\}
\end{equation}
Then $\P(\CA_2(J_j))\ge 1/2$ for all $J_j$, and the Markov property of the process ensures that $\CA_2(J_j)_{j\le m_k}$ are independent.
 Then Chernoff's bound yields that
\begin{equation}\label{eq:e3}
\begin{aligned}
    \P(\CA_3(v_i))&:=\P\big( \#\{j\le m_K: \CA_2(J_j) \mbox{ holds}\} \ge m_K/4 \big) \\
    &\ge \P\big(\mathrm{Bin}(m_K, 1/2)\ge m_K /4 \big) \ge 1- \e^{- c m_k },
    \end{aligned}
\end{equation}
for $c=1/48$.
Consider now $\{j: \CA_2(J_j)\}$, and for each such $j$, 
   call such $J_j$ \emph{successful} if there is some time $t\in J_j$ when at least $\lambda K^{1-\mu}/(4e)$ many leaves in the star-graph of $v_{i+1}$ are infected.
 We now lower bound the probability of the event that $J_j$ is successful conditioned on $\CA_2(J_j)$, as follows.
 Define a sequence of time-moments  $s_h:=\tau_j+h 4^\mu$ for $h\in\{1, \dots, \ell+1\}$,
and for $h=1,\dots, \ell$ we recursively check whether $u_h$ is infected at time $s_h$, given that $u_{h-1}$ is infected at $s_{h-1}$ (setting $u_0:=v_i$), and that whether $v_{i+1}=:u_{\ell+1}$ is infected at time $s_{\ell+1}$ given that $u_\ell$ is infected at time $s_\ell$. We also set $s_{\ell+2}:=s_{\ell+1}+1$ and check whether at least $\lambda K^{1-\mu}/(4e)$ many leaves in the star of $v_{i+1}$ are infected at time $s_{\ell+2}$, given that $v_{i+1}$ is infected at time $s_{\ell+1}$.  We shall thus bound, for some constant $c$, the time-interval lengths and their number as 
\begin{equation}\label{eq:tk}
t_K:=4^\mu (\ell+2)+2 \le (4^\mu\vee 2) (\ell+3), \qquad m_K=\lfloor T_K/t_K\rfloor \ge c \,T_K /\ell
\end{equation} 
Returning to an interval $J_j$ being successful, denote the infection status of the set of leaves in the star around $v_{i+1}$ by $\underline \xi^{(i+1)}_t$. Then, using the strong Markov property, we can lower bound
\begin{align}
\P&(J_j \mbox{ successful} \mid \CA_2(J_j
))\ge \P\big(  |\underline \xi^{(i+1)}_{s_{\ell+2}}|\ge \lambda K^{1-\mu}/(4e) \mid \xi_{\tau_j}(v_i)=1 \big)\label{eq:successful-def} \\
&\ge
\P(\xi_{s_1}(u_1)=1\mid \xi_{\tau_j}(v_i)=1 )\prod_{h=2}^{\ell+1}\P\Big( \xi_{s_h}(u_h) = 1\mid \xi_{s_{h-1}}(u_{h-1})=1\Big) \label{eq:product-factors} \\
&\qquad\cdot \P( |\underline \xi^{(i+1)}_{s_{\ell+2}}|\ge \lambda K^{1-\mu}/(4e)\mid \xi_{s_{\ell+1}}(v_{i+1})=1)\label{eq:first-infest}
\end{align}
On the last factor we shall use Claim \ref{claim:star} shortly, but first we bound the probability of each other factor in \eqref{eq:product-factors} from below by requiring that the sender vertex $u_{h-1}$ infects $u_{h}$ during a time interval of length $4^\mu$ from below, and then  $u_h$ stays infected for the rest of the time-interval. More generally, along an edge $(u,v)$, for any two time-moments $t<t'$, with infection rate $r$ along the edge,  
\[
\begin{aligned}
 \P(\xi_{t'}(v) = 1 \mid \xi_{t}(u) = 1  ) \ge \int_{\tau=0}^{t'-t} (\e^{-\tau})(r \e^{- r\tau}) \e^{-((t'-t)-\tau)}\mathrm d\tau  =\e^{-(t'-t)} \Big(1-\e^{-r (t'-t)}\Big).
 \end{aligned} 
\]
On the path $(u_0, u_1, u_2, \dots, u_\ell, u_{\ell+1})$ (with $u_0:=v_i$, $u_{\ell+1}:=v_{i+1}$), we apply this lower bound with $t'-t=4^\mu$ along each edge, with rates $r(u_{h-1}, u_{h})= \lambda/4^{\mu}$ for all $h\in\{2, \dots, \ell\}$, and $r(u_0, u_1)=r(u_\ell, u_{\ell+1})=\lambda/(2K)^{\mu}$.  
For \eqref{eq:first-infest}, we recall that $s_{\ell+2}-s_{\ell+1}=1$, so here \eqref{eq:star-i} directly applies, hence
\begin{equation}
\begin{aligned}
\P(J_j \mbox{ successful}\mid \CA_2(J_j))
&\ge \e^{-1}(1-\e^{-c_1 \la K^{1-\mu}}) \\
&\qquad \cdot \Big(\e^{-4^\mu} \big(1-\e^{-4^\mu\lambda/(2K)^{\mu}}\big)\Big)^2\prod_{h=1}^{\ell}\e^{-4^\mu} \Big(1-\e^{-4^\mu\cdot\lambda/4^{\mu}}\Big)
\end{aligned}
\end{equation}
Then we may apply that $1-\e^{-x}\ge x/2$ for all $x<1/2$ to arrive at
\begin{equation}\label{eq:qK}
\P(J_j \mbox{ successful}\mid \CA_2(J_j) ) \ge (1-\e^{-c_1 \la K^{1-\mu}}) e^{-4^\mu(\ell+2)-1} (\la/2)^{\ell} (2K)^{-2\mu}\ge c(c_2 \lambda)^{\ell}K^{-2\mu}=:q_{K},
\end{equation}
for some constant $c>0$ and $c_2:=\e^{-4^\mu}/2$, as long as $(1-\e^{-c_1 \la K^{1-\mu}})\ge 1/2$ which is ensured since we already assumed $K\ge K_0(\delta)$ at \eqref{eq:localtime}.
Since the time-intervals are disjoint, on $\CA_3(v_i)$ from \eqref{eq:e3}, by the strong Markov property, the indicators of the events $\{J_j \mbox{ successful}\} $ stochastically dominate $m_K/4$ independent trials (with $m_K$ from \eqref{eq:tk}), each with success probability $q_{K}$ from \eqref{eq:qK}. Let $\CA_4(v_i)$ be the event that at least one of the intervals is successful. Then
 \begin{equation}\label{eq:E2}
\P(\CA_4(v_i)\mid \CA_1(v_i)\cap \CA_3(v_i))  \ge 1- (1-q_K)^{m_K/4} \ge 1- \e^{-m_Kq_K/4},
 \end{equation}
 where we used that $1-x\ge \e^{-x/2}$ for all $x<1/4$, which is applicable since $q_K$ in \eqref{eq:qK} tends to $0$ with $K$. 
 We now analyze the exponent $m_Kq_K$ as a function of $K$ on the rhs of \eqref{eq:E2}.The assumption in this claim is that $\ell(K)=o(K^{1-2\mu})$ (in contrast to \eqref{eq:ellK} which is more specific). So, we may assume wlog that $\ell(K)$ can be written in the form 
 \begin{equation}\label{eq:ellK-new}
 \ell(K):=\wt g(K) K^{1-2\mu} \qquad \mbox{for}  \qquad \wt g(K)\to 0 \mbox{ as } K\to \infty.
 \end{equation}  
Recalling from \eqref{eq:star-iii} that $T_K=\exp(c_1 \lambda^2 K^{1-2\mu})$, and $m_K\ge cT_K/\ell(K)$ from \eqref{eq:tk}, as well as \eqref{eq:qK}, we obtain using that $1/\ell(K)\ge K^{-(1-2\mu)}$:
 \begin{equation} 
\begin{aligned}
 m_Kq_K&\ge  c  (T_K/\ell) \cdot  (c_2 \lambda)^{\ell}K^{-2\mu} = c\exp\bigg( c_1 \lambda^2 K^{1-2\mu} + \wt g(K) K^{1-2\mu} \log(c_2\lambda)\bigg) K^{-1}\\
 &=c \exp\bigg( \lambda^2 K^{1-2\mu} (c_1 - \wt g(K) |\log(c_2\la)|/\lambda^2 ) - \log (K)\bigg)
 \end{aligned}
 \end{equation}
 We now argue that for any small fixed $\lambda>0$ we can choose $K$ sufficiently large so that the rhs tends to infinity. 
 First choose $K(g, \lambda)$ so large that for all $K\ge K(g,\lambda)$ the inequality $\wt g(K)  |\log(c_2\lambda)|/\lambda^2 < c_1/2$ holds. This is doable since $\wt g(K)\to 0$. For all  $K>K(g,\lambda)$ we thus have 
 \[ m_Kq_K \ge C \exp\bigg( \lambda^2 K^{1-2\mu} c_1/2 - \log (K)\bigg) \]
 We now further increase $K(g, \lambda)$ if necessary so that 
 $ m_Kq_K\ge \log(8/\delta)/c.$ (We comment that by wlog assuming a monoton decreasing $\wt g$, the minimal $K({g, \lambda})$ can be chosen  constant multiple of $\wt g^{(-1)}\big( c_1 \lambda^2/ (2|\log (c_2\la)|)\big)\vee \lambda^{-(2+\varepsilon)/(1-2\mu)}$ for some $\eps>0$, for all $\lambda$ sufficiently small.) Returning to \eqref{eq:E2}, and using \eqref{eq:localtime}, \eqref{eq:e3} we see that 
 \[ \P(\CA_4(v_i)\mid \CA_3(v_i)\cap \CA_1(v_i))\ge 1-\delta/8 \quad \mbox{and}\quad \P(\CA_4(v_i)\cap \CA_3(v_i)\cap \CA_1(v_i)) \ge 1-\delta/2.\]
On the event $\CA_4(v_i)\cap \CA_3(v_i)\cap \CA_1(v_i)$, at least one $J_j$ is successful, and by \eqref{eq:successful-def}, that means that at least $\lambda K^{1-2\mu}/(4e)$ leaves in the star of $v_{i+1}$ are infected at some time in the interval $[t_0, t_0+T_K]$. Using the strong Markov property, and applying now \eqref{eq:star-iii}, $v_{i+1}$ stays $\lambda K^{-\mu}$ infested during the rest of the time interval $[t_0, t_0+T_K]$ with probability $1-\exp(-c_1\lambda^2K^{1-2\mu})\ge 1-\delta/4$ by our initial assumption that $K\ge K_0(\delta)$. This finishes the proof.  
\end{proof}

\subsubsection{Local survival through renormalization}\label{sec:renorm}
Having established Lemma \ref{lem:embedded_stars} and Claim \ref{claim:spread_between_stars} we are in a position to prove Theorems \ref{thm:prod_GW} and \ref{thm:max_GW}(a) by showing that the embedded structure $H_{K,\ell(K)}$ sustains the infection (locally) indefinitely with positive probability. This is formalized below in Lemma \ref{lem:survival_on_the_line}. The proof of this has two steps. The first step is a time-renormalization. Based on the results of Claim \ref{claim:spread_between_stars}, we prove that on $H_{K, \ell(K)}$ the infection moves between neighboring centers with large enough probability on a specified discrete time-scale, leading to a renormalized version of the contact process on $\N$. The second step is to establish a relationship between this renormalized contact process, and a certain oriented percolation model, which then can be analyzed by techniques from percolation theory, involving a Peierls-type argument. This connection was already used in \cite{DG83} to derive various results for the contact process on $\Z$.

\begin{lemma}\label{lem:survival_on_the_line}
For any fixed $\mu<1/2$ and $\lambda>0$, there is a $K_0(\lambda)$ such that the following holds for all $K>K_0(\lambda)$. Let $H=H_{K, \ell(K)}$ be the graph defined in Definition \ref{def:M-embedding} with $\ell(K)=o(K^{1-2\mu})$ and with $v_1$ being the center of its first star. Consider the penalty function $f(x,y)=(xy)^\mu$. Then both the contact process $\CPf(H,\ind_{v_1})$ and $\BRW(H,\ind_{v_1})$ exhibit local survival with positive probability.
\end{lemma}

\begin{proof} By the stochastic domination between $\CPf(H,\ind_{v_1})$ and $\BRW(H,\ind_{v_1})$ in Lemma \ref{lem:StochDom2}, it is enough to prove the statement for $\CPf(H,\ind_{v_1})$.
For fixed $\lambda>0$, we choose a small $\delta>0$ specified later. Then we choose $K$ large enough such that $K\ge K_{\lambda,\delta}$ as in Claim \ref{claim:spread_between_stars}. Finally, let $T_K=\exp(c_1\lambda^2 K^{1-2\mu})$ as in Claim \ref{claim:star}. Then, Claim \ref{claim:spread_between_stars} yields the following: for any $v_i$ in $H_{K,\ell(K})$, if $v_i$ is $\lambda K^{-\mu}$-infested at some time $t_0$, then $v_{i+1}$ is  $\lambda K^{-\mu}$-infested by $v_i$ at time $t_0+T_K$ with probability at least $1-\delta$, and the same holds for $v_{i-1}$ when $i\ge 2$. (However, these two events are not necessarily independent.) Throughout this proof, the term "infested" will refer to "$\lambda K^{-\mu}$-infested".

Now we construct an oriented percolation model, which we couple with $\CPf(H,\ind_{v_1})$ so that it dominates from below $\CPf(H,\ind_{v_1})$ restricted to the vertices $\{v_1,v_2,\ldots\}$ at times $\{T_K,2T_K,\ldots\}$. Let $\CH$ be an oriented graph on the vertex set
\begin{equation*}
V_{\CH}=\{(x,y)\in \Z^+\times\Z^+: x+y\text{ even}\}
\end{equation*}
with the oriented (equivalently, directed) edge set
\begin{equation}\label{eq:renorm_open}
E_{\CH}=\{((x_1,y_1),(x_2,y_1+1))\in V_{\CH}\times V_{\CH}: |x_2-x_1|=1\}.
\end{equation}
Observe that $\CH$ is isomorphic to a subgraph (a cone) of $\Z^+\times\Z^+$ as a graph but the edges are `diagonal' and have Euclidean length $\sqrt{2}$. In $\CH$, we will refer to the vertex sets $\{(x,1)\}_{x\in\Z^+}$ and $\{(1,y)\}_{y\in\Z^+}$ as the $x$- and $y$-axis, repectively. For every oriented edge $e=((x_1,y_1),(x_2,y_2))$ -- where $y_2=y_1+1$ and $x_2=x_1\pm 1$ by \eqref{eq:renorm_open} --  define the event $\CA_e=\CA_{(x_1,y_1),(x_2,y_2)}$ that either $v_{x_1}$ is not infested at time $y_1 T_K$, or $v_{x_1}$ is infested at time $y_1 T_K$ and it infests $v_{x_2}$ by time $y_2 T_K$ in the sense of Claim \ref{claim:spread_between_stars}. The same claim shows that
\begin{equation}\label{eq:renorm_open_prob}
\P(\CA_e)\ge 1-\delta \quad\text{for every }e\in E_{\CH}.
\end{equation}

Now let $\eta:V_{\CH}\to \{0,1\}$ be a function on the vertices of $\CH$ defined recursively as
\begin{equation}\label{eq:eta-def}
\eta((x,1))=\ind\{x=1\},\quad\quad
\eta((x,y+1))=
\begin{cases}
1 & \text{ if }\eta(x-1,y)=1 \text{ and }\CA_{(x-1,y),(x,y+1)} \text{ holds, or}\\
  & \quad \eta(x+1,y)=1 \text{ and } \CA_{(x+1,y),(x,y+1)} \text{ holds},\\
0 & \text{ otherwise}.
\end{cases}
\end{equation}
Define the event
\begin{equation}\label{eq:renorm_I1}
\CI_1=\{\text{$v_1$ is infested at time $T_K$ in $\CPf(H,\ind_{v_1})$}\},
\end{equation}
which exactly corresponds to $\eta((1,1))=1$.
Then, conditioned on $\CI_1$, $\eta(x,y)=1$ exactly when there is an ``infestation'' path $\pi$ through stars $(v_1=v_{\pi_1}, v_{\pi_2}, \dots, v_{\mathfrak{l}(\pi)}=v_x)$ so that $v_{\pi_j}$ is infested by $v_{\pi_{j-1}}$ at time $jT_K$. So, on $\CI_1$, 
\begin{equation}\label{eq:renorm_stochdom}
\big(\eta(x,y)\big)_{(x,y)\in V_{\CH}}\ {\buildrel d \over \le}\  \big(\xi_{y T_K}(v_x)\big)_{(x,y)\in V_{\CH}}.
\end{equation}
We now define a subgraph of $\CH$. Let us declare each edge $e\in E_{\CH}$ open if and only if $\ind\{\CA_e\}=1$,  closed otherwise, and denote the graph of open edges by $G(\CH)$. This is a percolation model, where the outgoing edges from a vertex $(x,y)$ are dependent, however, the outgoing edges from distinct vertices are independent due to the strong Markov property and Claim \ref{claim:spread_between_stars}.  The open connected component of $(1,1)$ is
\begin{equation}\label{eq:renorm_CCdef}
\CC_{(1,1)}=\{(x,y)\in V_{\CH}: \text{there is an oriented path of open edges from $(1,1)$ to $(x,y)$}\}.
\end{equation}
Then, comparing $\CC_{(1,1)}$ to $\{(x,y):\eta(x,y)\}=1\}$ in \eqref{eq:eta-def}, which is defined recursively as precisely those vertices that are accessible from $(1,1)$ via an oriented path of open edges in $\CH$, we obtain that $\{(x,y):\eta(x,y)\}=1\}=\CC_{(1,1)}$.

Now we carry out a Peierls-type argument to prove local survival of $\CPf$. Due to the coupling and stochastic domination in \eqref{eq:renorm_stochdom}, and \eqref{eq:renorm_CCdef}, it is enough to show that with positive probability $\CC_{(1,1)}$ contains infinitely many vertices of the form $(1,y)$. This implies for $\CPf$ that $v_1$ is infested at times $yT_K$, for infinitely many $y$, which guarantees local survival.
Let
\begin{equation}\label{eq:renorm_max}
Y_{\text{max}}=\sup\{y\in\Z^+:(1,y)\in\CC_{(1,1)}\}.
\end{equation}
We will prove that for small enough $\delta>0$ in \eqref{eq:renorm_open_prob} it holds that  $\P(Y_{\text{max}}=\infty)>3/4.
$

Assume to the contrary that $\{Y_{\text{max}}=k\}$ for some $k<\infty$. We now construct a path of length $k$, which starts from the $y$-axis next to $(1,k)$, and forms a part of the boundary of $\CC(1,1)$ containing enough closed edges in $\CH$. Define for each edge $e=((x_1,y_1),(x_2,y_2))\in E_{\CH}$ its (unoriented) dual $e'=\{(x_1,y_2),(x_2,y_1)\}$. The dual edges  connect vertices on the dual lattice $\CH':=\{(x,y)\in \Z^+\times\Z^+: x+y \text{ odd}\}$. We declare the dual edge $e'$ closed if $e$ is closed, and open if $e$ is open. We then define the (outer edge-) boundary of $\CC_{(1,1)}$ as the set of dual edges
\begin{equation}\label{eq:renorm_boundary}
\partial \CC_{(1,1)}=\{e':\text{ exactly one of the two endpoints of $e$ is in }\CC_{(1,1)}\}.
\end{equation}
Since $\CH$ is a cone in $\Z^+\times\Z^+$, and $\CC_{(1,1)}$ is connected per definition, $\partial\CC_{(1,1)}$ is a union of connected contours in $\CH'$, which along with (parts of) the $x$- and $y$-axes encircle $\CC_{(1,1)}$. Assume now that the event $\{Y_{\text{max}}=k\}$ occurs. This implies that  $(1,k)\in\CC_{(1,1)}$ and $(1,k+2)\notin\CC_{(1,1)}$. So, define the edges and their duals
\begin{align*}
\hat{e}_{k,1}&=((1,k),(2,k+1)),\qquad\quad \hat e_{k,1}'=\{(1,k+1), (2, k)\},\\
\hat{e}_{k,2}&=((2,k+1),(1,k+2)), \qquad \hat e_{k,2}'=\{(1,k+1), (2,k+2)\}.
\end{align*}
 Now, if $(2,k+1)\notin\CC_{(1,1)}$, then since $(1,k)\in \CC_{(1,1)}$, the dual edge $\hat{e}_{k,1}'\in\partial\CC_{(1,1)}$ (and  $\hat{e}_{k,2}'\notin\partial\CC_{(1,1)}$). In this case, define $\hat{e}_k=\hat{e}_{k,1}$. On the other hand, if $(2,k+1)\in\CC_{(1,1)}$, then since $(1,k+2)\notin \CC_{(1,1)}$, the dual edge  $\hat{e}_{k,2}'\in\partial\CC_{(1,1)}$ (and $\hat{e}_{k,1}'\in\partial\CC_{(1,1)}$). In this case, define $\hat{e}_k=\hat{e}_{k,2}$. In both of these cases, the vertex $(1,k+1)$ is the starting point of the dual $\hat{e}_k'$, which is in $\partial\CC_{(1,1)}$, and the other dual edge with endpoint $(1,k+1)$ is not in $\partial\CC_{(1,1)}$. Then we start exploring $\partial\CC_{(1,1)}$, starting from $e'_1:=\hat{e}_k'$ by following the dual edges in this connected component of $\partial\CC_{(1,1)}$. That is, the next dual edge in the path, denoted by $e'_2$, is incident to $(2,k)$ if $e'_1=\{(1,k+1),(2,k)\}$ and to $(2,k+2)$ if $e'_1=\{(1,k+1),(2,k+2)\}$. Then we continue from the other endpoint of $e'_2$, and so on. We continue this exploration process either indefinitely (if $\CC_{(1,1)}$ is infinite), or until we reach the $x$-axis (if $\CC_{(1,1)}$ is finite). As we explain next, these are the only two possible outcomes. For an example of the second outcome, see Figure \ref{fig:oriented}.

\begin{figure}[h]\label{fig:oriented}
\begin{center}
\includegraphics[scale=0.5]{oriented.pdf}
\caption{This example shows a finite oriented cluster of the origin $\CC_{(1,1)}$: filled black circles are vertices in $\CC_{(1,1)}$ while empty black circles are vertices that do not belong to $\CC_{(1,1)}$. The oriented, black edges are open in $\CH$, while the closed edges  of $\CH$ are not drawn. The red countour and red vertices belong to the dual lattice $\CH'$.
Since $Y_{\text{max}}=5$, the dual contour $\pi_\partial$ starts from $(1,6)$, and follows the closed dual edges colored red, ending at $(2,1)$. Edges of $\CH$ pointing out of $\CC_{(1,1)}$ are all closed (not drawn), whereas edges pointing into $\CC_{(1,1)}$ may be open -- such as the edge $((5,3),(4,4))$ -- or closed.}
\end{center}
\end{figure}
 
 Denote by $\pi_\partial=(e'_1,e'_2,\ldots)$ the path (as a sequence of dual edges) obtained this way. It is possible that $\pi_\partial$ visits the $y$-axis above $(1,k+1)$ (say at $(1,y')$ with $y'>k$), but since $Y_{\text{max}}=k$, this can only happen when $(2,y')\in \CC_{(1,1)}$ and $(1,y'+1)\notin \CC_{(1,1)}$, and then we can always continue the path $\pi_\partial$ by traversing the dual edge $\{(1,y'),(2,y'+1)\}$. 
 However, $\pi_\partial$ cannot visit the $y$-axis below $(1,k)$, since then we would have encircled the entire $\CC_{(1,1)}$, starting from $(1,k+1)$, without containing $(1,1)$, a contradiction. Hence, one of the two remaining cases happens. We either find an infinite path $\pi_{\partial}$ in $\partial\CC_{(1,1)}$, and then we set $\pi_\partial(k)$ to be the sequence of its first $k$ edges. Or, we find a finite path $\pi_{\partial}$ that reaches the $x$-axis, in particular, the dual vertex $(2, 1)$. This path has length at least $k$, since the path starts at $(1,k+1)$, and the $y$ coordinate only  changes by $\pm1$ between consecutive vertices on the path. In this case we again set $\pi_\partial(k)$ to be the sequence of the first $k$ edges of $\pi_\partial$.
 
We now categorize edges of $\pi_\partial(k)$ (all are in $\partial \CC_{(1,1)}$) as follows. 
Recall that edges of $\CH$ in \eqref{eq:renorm_open} are oriented (directed), and recall 
\eqref{eq:renorm_boundary}. Given $\CC_{(1,1)}$ let us call the dual edge $e'\in \partial \CC_{(1,1)}$ an \emph{outward} dual edge, if for the edge $e=((x_1,y_1),(x_2,y_2))$ it holds that $(x_1, y_1)\in \CC_{(1,1)}$ and $(x_2, y_2)\notin \CC_{(1,1)}$ and let us call $e'$ an \emph{inward} dual edge if $(x_1, y_1)\notin \CC_{(1,1)}$ and $(x_2, y_2)\in \CC_{(1,1)}$. Per definition of $\CC_{(1,1)}$ in \eqref{eq:renorm_CCdef}, the outward edges and their duals are all closed. However, $\CC_{(1,1)}$ does not determine the status of inward dual edges. 

We now prove that for any realization of $\CC_{(1,1)}$, at least half of the edges of $\pi_\partial(k)$ are outward dual edges, and hence closed.
Let us introduce the notation $\pi_0=(1,k+1), \pi_1, \pi_2, \dots, \pi_k, \dots$ for the vertices of the path $\pi_\partial$ in order, and define the directed edge $\underline{e}'_i=(\pi_{i-1}, \pi_i)$ for all $i\ge 1$ (the directed version of $e'_i$). Then for all outward dual edges $e'_i\in\pi_\partial$, $\underline{e}'_i$ is pointing to the right (in the direction of increasing $x$ coordinate), and for all inward dual edges $e'_i\in\pi_\partial$, $\underline{e}'_i$ is pointing to the left (in the direction of decreasing $x$ coordinate).
Since $\pi_\partial(k)$ starts from $(1,k+1)$, which is part of the $y$-axis, and remains in the positive quadrant, at least half of its dual edges have to be directed to the right, thus, duals of outward edges. Hence, at least $k/2$ dual edges in $\pi_\partial(k)$ are closed. Further, since every vertex in $V_{\CH}$ has at most two outgoing (non-dual) edges, in every possible realization $(e_1', e_2', \dots, e_k')$ of $\pi_{\partial}(k)$ we can find $k/4$ edges that are all closed and that their oriented non-dual edges in $\CH$ all start from different vertices. 


By \eqref{eq:renorm_open_prob}, the probability that a given edge (and its dual) is closed is at most $\delta$. As mentioned before \eqref{eq:renorm_CCdef}, the status of different edges are not independent, however, $\CA_{(x_1,y_1),(x_2,y_2)}$ is independent of $\CA_{(x'_1,y'_1),(x'_2,y'_2)}$ if $(x_1,y_1)\ne(x'_1,y'_1)$. That is, two edges $e_1,e_2\in E_\CH$ are open or closed independently if their starting points are distinct. 

We call a given connected path $(e'_1,\ldots,e'_k)$ of dual edges eligible if it is a possible realization of $\pi_\partial(k)$ (of which one requirement is that one of the endpoints of $e_1'$ is $(1,(k+1))$). Then, for all such $(e_1', e_2', \dots, e_k')$, 
\begin{equation}\label{eq:renorm_path_prob}
\P\big(\pi_\partial(k)=(e'_1,\ldots,e'_k)\big)\le \delta^{k/4}.
\end{equation}
Next, we upper bound the number of eligible paths $(e'_1,\ldots,e'_k)$. Since $(e'_1,\ldots,e'_k)$ is a path starting from $(1,k+1)$ on the dual lattice $\CH'$ isomorphic to a quadrant of $\Z^2$, each of the $k$ steps in the exploration of $\pi_\partial(k)$ can be taken in one of at most three directions. This yields that the number of possible trajectories is at most $3^k$. Therefore, by a union bound, 
\begin{equation}\label{eq:renorm_Yk_prob}
\P(Y_{\text{max}}=k)\le \P\Big(\bigcup_{(e_1', \dots, e_k') \text{ eligible}} \{\pi_\partial(k)=(e_1', \dots, e_k')\}\Big)\le 3^k\delta^{k/4}.
\end{equation}
Then \eqref{eq:renorm_Yk_prob} implies that
\begin{equation}\label{eq:renorm_Ak_prob}
\P(Y_{\max}<\infty)=\sum_{k=1}^\infty\P(Y_{\text{max}}=k)\le \sum_{k=1}^\infty 3^k\delta^{k/4}<1/4,
\end{equation}
whenever $\delta\in(0, (1/15)^4)$.
Consequently, 
$\P(Y_{\text{max}}=\infty)>3/4.$
Finally, recalling $\CI_1$ from \eqref{eq:renorm_I1},  $\P(\CI_1)>1/3$ for large enough $K$ by Claim \ref{claim:star}.  By the stochastic dominance in \eqref{eq:renorm_stochdom}, it follows from a union bound that
\begin{equation}\label{eq:renorm_local_survival}
\P\big(\CPf(H,\ind_{v_1})\text{ survives locally at }v_1\big)\ge \P\big(\CI_1\cap \{Y_{\text{max}}=\infty\}\big) \ge 1-2/3-1/4>0. 
\end{equation}
 This proves local survival of $\CPf(H,\ind_{v_1})$ with positive probability.
\end{proof}

\begin{proof}[Proof of Theorems \ref{thm:prod_GW} and \ref{thm:max_GW}(a)]
Lemma \ref{lem:embedded_stars} states that for some $M\ge 1$ there exists $K_1$ such that and for $K>K_1$ and $\ell(K)$ as in \eqref{eq:ellK} $H_{K,\ell(K)}$ can be $M$-embedded in $\CT$ almost surely. Set $\bar\lambda=\lambda/M^{2\mu}$ and let $K_0(\bar\lambda)$ be given by Lemma \ref{lem:survival_on_the_line}. Now let
$K>\max(K_0(\bar\lambda),K_1)$. Then Lemma \ref{lem:embedded_stars} yields that $H_{K,\ell(K)}$ can be $M$-embedded in $\CT$ almost surely. Let $v_1$ be the center of the first star in the embedded $H_{K,\ell(K)}$. Recalling \eqref{eq:factor-M} in Definition \ref{def:M-embedding}, we observe that the process $\CPf(\CT,\ind_{v_1})$ restricted to the vertices of the embedded $H_{K,\ell(K)}$ is stochastically dominated from below by the process $\mathrm{CP}_{f,\bar\lambda}(H_{K,\ell(K)},\ind_{v_1})$ on a standalone copy of $H_{K,\ell(K)}$. Combining this with Lemma \ref{lem:survival_on_the_line} and $K\ge K_0(\bar\lambda)$ implies that $\mathrm{CP}_{f,\bar\lambda}(H_{K,\ell(K)},\ind_{v_1})$ survives locally with positive probability. This, along with the fact that with positive probability, $\CPf(\CT,\ind_\varnothing)$ infects $v_1$ at some point in time finishes the proof.
\end{proof}
